Accelerating Smooth Games by Manipulating Spectral Shapes

We use matrix iteration theory to characterize acceleration in smooth games. We define the spectral shape of a family of games as the set containing all eigenvalues of the Jacobians of standard gradient dynamics in the family. Shapes restricted to the real line represent well-understood classes of problems, like minimization. Shapes spanning the complex plane capture the added numerical challenges in solving smooth games. In this framework, we describe gradient-based methods, such as extragradient, as transformations on the spectral shape. Using this perspective, we propose an optimal algorithm for bilinear games. For smooth and strongly monotone operators, we identify a continuum between convex minimization, where acceleration is possible using Polyak's momentum, and the worst case where gradient descent is optimal. Finally, going beyond first-order methods, we propose an accelerated version of consensus optimization.

==> snd_figure_geometric.tex <==
\begin{figure}
    \centering
    \setcounter{t}{80}
    \setcounter{L}{10}
    \hspace{-4mm}
    \begin{tikzpicture}[scale=0.65]
        \begin{axis}[
            grid=major,
            %From https://tex.stackexchange.com/questions/61039/how-to-keep-a-11-scale-with-x-and-y-axis
            axis equal image,
            yticklabel={
            $\pgfmathprintnumber{\tick}i$
            },
        	xmin=0,   xmax={\value{L} + 2},
        	ymin={-\value{L} - 1},   ymax={\value{L} + 1},
        	]
           \draw [domain=-\value{t}:\value{t}, draw=yellow, thick, fill=yellow!50!white, fill opacity=0.5, samples=65] plot (axis cs: {\value{L}*cos(\x)}, {\value{L}*sin(\x)});
           \draw [draw=yellow, thick](axis cs: {\value{L}*cos(\value{t})}, {\value{L}*sin(\value{t})}) -- (axis cs: {\value{L}*cos(\value{t})}, {\value{L}*sin(-\value{t})});
           \draw [domain=-180:180, draw=red, fill=red!50!white, thick, fill opacity=0.5, samples=65] plot (axis cs: {\value{L}*(1 + cos(\value{t}))/2 + cos(\x) * \value{L}*(1 - cos(\value{t}))/2}, {sin(\x) * \value{L}*(1 - cos(\value{t}))/2});
           \node[anchor=south east] (mu) at (axis cs: {\value{L} * cos(\value{t})}, 0) {$\mu$};
           \draw [fill=black] (axis cs: {\value{L} * cos(\value{t})}, 0) circle (1pt);
           \node [circle, anchor=south west] (L) at (axis cs: {\value{L}}, 0) {$L$};
           \draw [fill=black] (axis cs: {\value{L}}, 0) circle (1pt);
       \end{axis}
    \end{tikzpicture}
    \hspace{-3mm}
    \newcounter{mu}
    \setcounter{mu}{2}
    \setcounter{L}{28}
    \begin{tikzpicture}[scale=0.65]
        \begin{axis}[
            grid=major,
            %From https://tex.stackexchange.com/questions/61039/how-to-keep-a-11-scale-with-x-and-y-axis
            axis equal image,
            yticklabel={
            $\pgfmathprintnumber{\tick}i$
            },
        	xmin=0,   xmax={\value{L} + 2},
        	ymin={-\value{L}/2},   ymax={\value{L}/2},
        	]
           \draw [domain=-180:180, thick, draw=blue, fill=blue!50!white, fill opacity=0.5, samples=65] plot (axis cs: {(\value{L} + \value{mu})/2 + cos(\x) * (\value{L} - \value{mu})/2}, {sin(\x) * sqrt(\value{mu}*\value{L})});
           \draw [domain=0:1, thick, draw=blue!80!white] plot (axis cs:{(\x * \value{mu} + (1 - \x) * \value{L}}, 0);
           \draw [domain=-1:1, thick, draw=blue!80!white] plot (axis cs:{0.5 * (\value{mu} + \value{L})},{\x * sqrt(\value{mu}*\value{L})});
            \node[anchor=south east] (mu) at (axis cs: {\value{mu}}, 0) {$\mu$};
           \draw [fill=black] (axis cs: {\value{mu}}, 0) circle (1pt);
           \node [anchor=south west] (L) at (axis cs: {\value{L}}, 0) {$L$};
           \draw [fill=black] (axis cs: {\value{L}}, 0) circle (1pt);
           \node [anchor=west] (epsilon) at (axis cs:{0.5 * (\value{mu} + \value{L})},{0.5 * sqrt(\value{mu}*\value{L})}) {\textcolor{blue}{$\epsilon$}};
        \end{axis}
    \end{tikzpicture}
    \hspace{-4mm}
    \caption{\textbf{Left:} Illustration of the proof of \cref{cor: lb strongly monotone}. The yellow set correspond to $K$, the set of strongly monotone problems while the red disc is the disc of center $\frac{1}{2}(\mu + L)$ and radius $\frac{1}{2}(L- \mu)$ which fits inside.
    \textbf{Right:} Illustration of $K_\epsilon$ of \cref{prop: perturbed acceleration} with $\epsilon = \sqrt{\mu L}.$
    \varvspace{-2ex}
    }\label{figure: visual proof lb}
\end{figure}
